Polynomial Logical Zonotope: A Set Representation for Reachability Analysis of Logical Systems

In this paper, we introduce a set representation called polynomial logical zonotopes for performing exact and computationally efficient reachability analysis on logical systems. We prove that through this polynomial-like construction, we are able to perform all of the fundamental logical operations (XOR, NOT, XNOR, AND, NAND, OR, NOR) between sets of points exactly in a reduced space, i.e., generator space with reduced complexity. Polynomial logical zonotopes are a generalization of logical zonotopes, which are able to represent up to $2^n$ binary vectors using only $n$ generators. Due to their construction, logical zonotopes are only able to support exact computations of some logical operations (XOR, NOT, XNOR), while other operations (AND, NAND, OR, NOR) result in over-approximations in the generator space. In order to perform all fundamental logical operations exactly, we formulate a generalization of logical zonotopes that is constructed by dependent generators and exponent matrices. While we are able to perform all of the logical operations exactly, this comes with a slight increase in computational complexity compared to logical zonotopes. To illustrate and showcase the computational benefits of polynomial logical zonotopes, we present the results of performing reachability analysis on two use cases: (1) safety verification of an intersection crossing protocol and (2) reachability analysis on a high-dimensional Boolean function. Moreover, to highlight the extensibility of logical zonotopes, we include an additional use case where we perform a computationally tractable exhaustive search for the key of a linear feedback shift register.

==> 6-reach_cont.tex <==

\subsection{Reachability Analysis for Continuous-Time Systems}

%To do, I think
%\begin{itemize}
%\item Introduce why this is a very interesting problem (discrete time measurements, but system continuous time)
%\item Introduce exact discretization (+ assumptions, if applicable)
%\item Explain the logm operator + its series calculation
%\item Motivate why this is a hard problem
%\item State assumption
%\item State Theorem + Proof
%\item Short remark that calculating the series with the zonotope is also possible with guaranteed approximation error, but numerics have shown that the results are overly conservative?
%\end{itemize}

We are interested in computing the reachable sets of continuous time systems that are consistent with the data sampled in discrete time. Consider the following state space
\begin{align}
    \dot{x}(t) = A_c x(t) + B_c u(t) + w(t). 
    \label{eq:syscont}
\end{align}

%Measuring the current is type of measuring the derivativeof the voltage of the capacitor. Also, measuring the voltage of the inductor is kind of measuring the derivative of the current. The accelerometer sensor is measuring the derivative of the velocity as well. This approach can be summarized in the following theorem and is useful in certain applications. 

We propose two approaches to compute these reachable sets. First approach requires collecting the derivative of the signal as done in \cite{conf:contin1,conf:contin2,conf:contin3} and one example for that is the accelerator sensor. If we consider sampled noisy state derivative $\tilde{\dot{x}}(k)$ and noisy state, i.e.,
\begin{align}
\tilde{\dot{x}}(k) = \dot{x}(k) + g(k),\\
\tilde{x}(k) = x(k) + v(k),
\end{align}

where $g(k) \in \mathcal{Z}_g=\zono{c_g,G_g}$ and $v(k) \in \mathcal{Z}_v$ are bounded measurement noise. We collect $T$ data points  
\begin{align*}
    \tilde{\dot{X}} &:= \begin{bmatrix} \tilde{\dot{x}}(0) & \tilde{\dot{x}}(1) & \dots & \tilde{\dot{x}}(T-1) \end{bmatrix},
\end{align*}
with noise
\begin{align*}
 \hat{G} &:= \begin{bmatrix} \hat{g}(0) & \hat{g}(1) & \dots &\hat{g}(T-1) \end{bmatrix}.
\end{align*}

Similar to before, we have the noise in the collected data within a matrix zonotope, i.e., $G \in \mathcal{M}_g =\zono{C_{\mathcal{M}_g},G_{\mathcal{M}_g}^{(1:T)}}$. The problem is close the noisy measurement for discrete system with additional noise $g(k) \in \mathcal{Z}_g$ that affects the derivative of the data. We have for specific data points with actual noise $\hat{g}(k)$, $\hat{v}(k)$ and $\hat{w}(k)$:

\begin{align}
    (\tilde{\dot{X}})_i - \hat{g}(k) = \begin{bmatrix} A_c & B_c \end{bmatrix} \begin{bmatrix} (\tilde{X}_-)_i \\ (U)_i \end{bmatrix} - A_c \hat{v}(k) + w(k).
\end{align}

Again we first fit a model $M_c$ while neglecting the term $A_c \hat{v}(k)$ using least square as follows:
\begin{align}
    M_c = (\tilde{X}_+ - C_{\mathcal{M}_g} - C_{\mathcal{M}_w}  ) D_c
    \label{eq:Mc}
\end{align}
where 
 \begin{align}
    \begin{bmatrix} 
    \tilde{X}_{-} \\ U_{-} 
    \end{bmatrix} D_c = I,
    \label{eq:cond2Mc}
\end{align}
Then we find a zonotope $\mathcal{Z}_d$ that bounds the term $AV_-$ and the model mismatch, with the assumption  that the data is informative enough, as follows

\begin{align}
    \mathcal{M}_d &=\dot{X} - \mathcal{M}_w - \mathcal{M}_g - M_c \begin{bmatrix}X_{-} \\ U_{-} \end{bmatrix}.\label{eq:zc}
    \end{align}
Then obtain the upper and lower bound in a zonotope $\mathcal{Z}_d$ from $\mathcal{M}_d$ as in \eqref{eq:argmaxMAV} and \eqref{eq:argminMAV}.  
    
%    \begin{align}
%[\underline{\mathcal{M}}_d , \overline{\mathcal{M}}_d ]&= \text{intervalMatrix}(\mathcal{M}_d),\\
%(\overline{\mathcal{Z}_d})_i &= \argmaxB_j{(\overline{\mathcal{M}}_d)_{i,j}}, \\ (\underline{\mathcal{Z}_d})_i &= \argminB_j{(\underline{\mathcal{M}}_d)_{i,j}}, \\
%\mathcal{Z}_d &= \text{zonotope}(\underline{\mathcal{Z}}_d,\overline{\mathcal{Z}}_d). 
%\end{align}

Let $M_c =\begin{bmatrix} A_{M_c} & B_{M_c} \end{bmatrix}$. Then the next step is to use one of the readability analysis tool to find the reachable sets using the following parameters ($A_t$, $B_t$, $\mathcal{U}_t$, $\mathcal{X}_{t,0}$)
\begin{align}
 A_t &= A_{M_c}\\
 B_t & = 1 \\
 \mathcal{X}_{t,0} &= \mathcal{X}_{0} \\
 \mathcal{U}_t &= B_{M_c} \mathcal{U} + \mathcal{Z}_w +\mathcal{Z}_d
\end{align}

We consider the $\mathcal{Z}_w +\mathcal{Z}_d$ in $\mathcal{U}_t$ to be integrated along with the input. 

%\begin{theorem}
%Consider collected sampled data $\mathcal{D}$ from the system \eqref{eq:syscont}, the data-driven reachable set can be computed using traditional reachable techniques with the following parameters ($\mathcal{U}_c,\mathcal{A}_c,\mathcal{B}_c$)
%\begin{align}
% \mathcal{A}_c &= \mathcal{A}_{\Sigma,c}'\\
% \mathcal{B}_c & = 1 \\
% \mathcal{U}_c &= \mathcal{B}_{\Sigma,c}' \mathcal{U} + \mathcal{Z}_w +\mathcal{Z}_d
%\end{align}
%where
%\begin{align}
%\begin{bmatrix} 
%    X_- \\ U_- 
%\end{bmatrix} H &= I
%\end{align}
%\begin{align}
%\mathcal{M}_{\Sigma,c}' &= (\dot{X}_- - \mathcal{M}_w) H\\
%[ \mathcal{A}_{\Sigma,c}', \mathcal{B}_{\Sigma,c}'] &= \mathcal{M}_{\Sigma,c}'\\
%\mathcal{M}_d &=\dot{X}_- - \mathcal{M}_w - \mathcal{M}_{\Sigma,c} \begin{bmatrix}X_{-} \\ U_{-} \end{bmatrix},\label{eq:zc}\\
%[\overline{\mathcal{M}}_d , \underline{\mathcal{M}}_d ]&= \text{intervalMatrix}(\mathcal{M}_d),\\
%\overline{\mathcal{Z}_d}(i) &= \argmaxB_j{\overline{\mathcal{M}}_d(i,j)}, \\ \underline{\mathcal{Z}_d}(i) &= \argminB_j{\underline{\mathcal{M}}_d(i,j)}, \\
%\mathcal{Z}_d &= \text{zonotope}(\overline{\mathcal{Z}_d},\underline{\mathcal{Z}_d}), 
%\end{align}
%\end{theorem}



We propose another approach for data-driven reachability analysis for continuous time systems without requiring collecting the derivatives of the states. First of all, we assume that the discrete-time data points are obtained through zero-order hold inputs, which is the case in many application scenarios. Our approach is based on converting all the possible $\begin{bmatrix} A & B\end{bmatrix}$ in discrete time to continuous time. First we convert $\mathcal{M}_\Sigma$ to interval matrix which then bounds the all possible $\begin{bmatrix} A & B\end{bmatrix}$ as follows
\begin{align}
    [\underline{\mathcal{M}}_\Sigma,\overline{\mathcal{M}}_\Sigma ]&= intervalMatrix(\mathcal{M}_\Sigma) 
\end{align} 
 \begin{align}
   \underbrace{\begin{bmatrix}\underline{A} & \underline{B}\\ 0 & I\end{bmatrix}}_{\underline{D}} \leq \begin{bmatrix} A & B \\ 0 & I\end{bmatrix} \leq \underbrace{\begin{bmatrix} \overline{A} & \overline{B}   \\ 0 & I\end{bmatrix}}_{\overline{D}}
\end{align}  
where the operation $\leq$ is element wise. Let $\overline{D} = C_d + \Delta D_u$  and $\underline{D} = C_d - \Delta D_l$ where $C_d$ is any matrix between the bounds, i.e., $\underline{D} \leq C_d \leq \overline{D}$. The following theorem bounds all the possible $\begin{bmatrix} A_c & B_c\end{bmatrix}$ as follows: 

%Let $D_c :=  \begin{bmatrix} A_c & B_c \\ 0 & I\end{bmatrix}$, 

\begin{theorem}
Given the lower bounds $\begin{bmatrix}\underline{A} & \underline{B}\end{bmatrix}$ and upper bounds $\begin{bmatrix}\overline{A} & \overline{B}\end{bmatrix}$ on $\begin{bmatrix}A & B\end{bmatrix}$, we can bound $\begin{bmatrix}A_c & B_c\end{bmatrix}$ as follows
\begin{align}
   \begin{bmatrix} \underline{A}_c & \underline{B}_c \\ 0 & I\end{bmatrix} \leq  \begin{bmatrix} A_c & B_c \\ 0 & I\end{bmatrix}  \leq \begin{bmatrix} \overline{A}_c & \overline{B}_c \\ 0 & I\end{bmatrix}
\end{align}
\begin{align}
\begin{bmatrix} \overline{A}_c & \overline{B}_c \\ 0 & I\end{bmatrix} T_s&= \max(\log\begin{bmatrix} \overline{A} & \overline{B} \\ 0 & I\end{bmatrix},\log\begin{bmatrix} \underline{A} & \underline{B} \\ 0 & I\end{bmatrix})\\
\begin{bmatrix} \underline{A}_c & \underline{B}_c \\ 0 & I\end{bmatrix}T_s &= \min(\log\begin{bmatrix} \overline{A} & \overline{B} \\ 0 & I\end{bmatrix},\log\begin{bmatrix} \underline{A} & \underline{B} \\ 0 & I\end{bmatrix}),
\end{align}
where $T_s$ is the sampling time, $0 \leq \Delta D_l \leq 1$, $0 \leq\Delta D_u \leq 1$, $\Delta D_l \leq (C_d-I)$, $\Delta D_u \leq (C_d-I)$, and $C_d - I \leq 1$. The log is the matrix logarithm. The max, min and less than are element wise. 
\end{theorem}




\begin{proof}
We aim to prove that we can still bound $\begin{bmatrix} A_c & B_c \end{bmatrix}$ given the bounds in discrete time. Taking the logarithm of a matrix of $C_d$ and represented by power series.
\begin{align}
     log(C_d) &= \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(C_d - I)^k}{k}. \label{eq:cd}    %(C_d - I) - \frac{(C_d - I)(C_d - I)^T}{2}  +\dots
\end{align}
Considering $log(C_d +\Delta D)$ results in 
\begin{align}
log(C_d +\Delta D_u) =& \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(C_d  - I +\Delta D_u)^k}{k}\nonumber\\
=&  \sum_{k=1}^{\infty} \frac{(-1)^{k+1}}{k} \sum_{i=0}^{i}{k \choose i} (C_d  - I )^{k-i}\Delta D_u^i \label{eq:cddeltad}
%log(C_d +\Delta D) =& C_d +\Delta D - I - 0.5(C_d +\Delta D - I)^2 \nonumber\\
%&+ \frac{(C_d +\Delta D - I)^3}{3} - \frac{(C_d +\Delta D - I)^4}{4} + \dots \nonumber\\
%=&  C_d +\Delta D - I - 0.5 (C_d - I)^2 \nonumber\\
% - \Delta D (C_d  - I) - &0.5  \Delta D^2  + \frac{(C_d  - I)^3}{3} +  \Delta D(C_d  - I)^2 \nonumber\\ 
%+  \Delta D^2(C_d  - I) +& \frac{\Delta D^3}{3} - 0.25(C_d  - I)^4 - (C_d  - I)^3\Delta D \nonumber\\
%- 1.5(C_d  - I)^2&\Delta D^2 -  (C_d  - I)\Delta D^3 - 0.25 \Delta D^4 + \dots
\end{align}
Subtracting \eqref{eq:cd} from \eqref{eq:cddeltad} with denoting $h(\Delta D_u)= log(C_d +\Delta D_u) -  log(C_d)$ results in
\begin{align}
  h(\Delta D_u)\! =&\!\! \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k} \bigg(\! \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}\Delta D_u^i\! \nonumber\\ 
  &+ (C_d  -\! I )^k\! \bigg) -  \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k} (C_d  - I )^k \nonumber\\
   =& \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k}  \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}\Delta D_u^i\!
\end{align}
Similarly, we can find $h(-\Delta D)$ as
\begin{align}
h(-\Delta D_l)\! =  \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k}  \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}(-\Delta D_l)^i
\end{align}
Bounding the system dynamics in continuous time can be done by making sure that both $h(\Delta D_u)$ and $h(-\Delta D_l)$ do not increase or decrease together but one increases and the other decreases. 
%\begin{align}
%log(C_d + \Delta D) - log(C_d)&= \Delta D - \Delta D(C_d  - I) - 0.5\Delta D^2 \nonumber\\
%+ \Delta D (C_d  - I)^2 +&  (C_d  - I)\Delta D^2 + \frac{\Delta D^3}{3} \nonumber\\
%- (C_d  - I)^3\Delta D -& 1.5(C_d  - I)^2\Delta D^2 - (C_d  - I)\Delta D^3 \nonumber\\
%- \Delta D^4 + \dots&\\
%log(C_d - \Delta D) - log(C_d)&= -\Delta D + \Delta D(C_d  - I) - 0.5\Delta D^2 \nonumber\\
%- \Delta D (C_d  - I)^2 +&  (C_d  - I)\Delta D^2 - \frac{\Delta D^3}{3} \nonumber\\
%+ (C_d  - I)^3\Delta D -& 1.5(C_d  - I)^2\Delta D^2 + (C_d  - I)\Delta D^3 \nonumber\\
%- \Delta D^4 + \dots&
%\end{align}
Given that $0 \leq \Delta D_u \leq 1$, $0 \leq \Delta D_l\leq 1$ and $(C_d-I) \leq 1$, then the dominant terms are $\Delta D_u$ and $\Delta D_u(C_d  - I)$ (similarly with $\Delta D_l$) and they are with different signs for $h(\Delta D_u)$ and $h(-\Delta D_l)$. At odd  value of index $i$, the $h(\Delta D_u)$ and $h(-\Delta D_l)$ have difference sign which support our claim. For index $i$ equals even values, both $h(\Delta D_u)$ and $h(-\Delta D_l)$ have the same sign. However given that $\Delta D_l \leq (C_d-I)$ and $\Delta D_u \leq (C_d-I)$, then there is always a term at the same index $i$ with greater value. %For instance, the terms $(C_d  - I)\Delta D^2$, $1.5(C_d  - I)^2\Delta D^2$, and $\Delta D^4$ are smaller than the comparable terms in the series.  
\end{proof}





%Assume that even though we have discrete-time trajectories, the underlying system is in fact continuous time. To retrieve a reachability analysis also in between data points, we are therefore interested in finding a set of continuous time systems that are consistent with the data.

%First of all, we assume that the discrete-time data points are obtained through zero-order hold inputs, which is the case in many application scenarios. % (note: realistic assumption on actuator). (Remark: This could also be refined to ramp-invariant transformation)





%Second assumption, we assume that the sampling rate is satisfactory and the spectral norm of $AT_s $ satisfies the following inequality:
%\begin{align*}
%   \| A T_s \| \leq 0.5
%\end{align*}

%Then we know 
%\begin{align*}
%    A_{\mathrm{disc}} &= e^{AT_s} = I + AT_s + \frac{1}{2!}(A T_s)^2 + \dots \\
%    B_{\mathrm{disc}} &= \int_0^{T_s} e^{At} B dt = \left( I T_s + A T_s^2 + \frac{1}{2!}A^2 T_s^3 + \dots \right) B
%\end{align*}

%\begin{theorem}
%The approximation error can be bounded by 
%\begin{align*}
%    \| E_m \| \leq \frac{\rho (L) ^{m+1}}{(m+1)(1+\rho(L))}
%\end{align*}
%where $\rho(L)$ denotes the spectral radius of $L$.
%\end{theorem}
%\begin{proof}
% (Lastman, Puthenpura and Sinha 1984)
%\end{proof}

%\subsubsection*{Algorithm \cite{conf:bookdisc2cont}}
%\begin{enumerate}
%    \item Determine $L = A_{\mathrm{disc}} - I$.
%    \item Set $D^{(1)} = I$, $M^{(1)} = I$ and $i=1$.
%    \item Perform the following computations recursively
%    \begin{align*}
%        M^{(i+1)} &= \frac{-i L M^{(i)}}{i+1} \\
%        D^{(i+1)} &= D^{(i)} + M^{(i+1)} \\
%        i &= i+1
%    \end{align*}
%    until $i=m$.
%    \item Finally, $AT = DL$, $BT = D B_{\mathrm{disc}}$
%\end{enumerate}



% This is what we need!
% https://link.springer.com/content/pdf/10.1007%2F978-94-011-3558-0.pdf p.131

%A method to calculate \cite{conf:disc2cont}, but calculations are involved and not tractable for matrix zonotopes. However, we can calculate the Euler approximation and then bound the local truncation error?

% Can we use this? "TRANSFORMATION OF CONTINUOUS-TIME MODEL OF A LINEAR MULTIVARIABLE SYSTEM FROM ITS DISCRETE-TIME MODEL"

%\tb{no results here - just thoughts we can discuss}
%$\rightarrow$ How can we find the continuous time state space description?
%Assuming zero-order hold for the input (I think a good choice), we retrieve
%\begin{align*}
%    A_{\text{disc}} = e^{AT_s}
%\end{align*}
%with $T_s$ being the sampling time. However, calculating the logarithm of a matrix is usually done via diagonalization. If $\|A_{\text{disc}} - I \| < 1$ (what does that mean for us?), then it can be calculated the following series converges:
%\begin{align*}
%    A T_s = \log (A_{\mathrm{disc}}) = \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(A_{\mathrm{disc}} - I)^k}{k}
%\end{align*}
%..can we calculate this sum via Zonotopes? We can only be approximating the true matrix.

%..which is actually the Euler integration. For small timesteps $T_s$, $e^{A T_s} \approx I + A T_s $, i.e. $A T_s \approx A_{\mathrm{disc}} - I  \left( = \sum_{k=1}^{1} (-1)^{k+1} \frac{(A_{\mathrm{disc}} - I)^k}{k}\right)$, $B T_s \approx B_{\mathrm{disc}}$. % $D_{\mathrm{disc}} = D$, $C_{\mathrm{disc}} = C$
% http://eceweb1.rutgers.edu/~gajic/solmanual/slides/chapter8_DIS.pdf
% https://homes.esat.kuleuven.be/~maapc/static/files/CACSD/Slides/chapter2.pdf

%I guess we can use Euler discretization for small timesteps - but we introduce an error. Can we bound the error? Then we could add this error in the reachability analysis. 

%The local error (error per step) is proportional to the square of the step size.
%Assume $x$ has a continuous second derivative. Local truncation error LTE:
%\begin{align*}
%    \mathrm{LTE} = \frac{1}{2} T_s^2 M 
%\end{align*}
%where $M$ is the an upper bound on the second derivative of $x$ on the given interval $[t_0, t_0 + h]$.

%\begin{align*}
%    \dot{x} &= Ax + Bu \\
%    \ddot{x} &= A \dot{x} = A^2 x + ABu
%\end{align*}
%While we cannot calculate the exact discretization error, we can approximate it by $A_{\mathrm{disc}}^2 x(t_0) + A_{\mathrm{disc}} B_{\mathrm{disc}} u(t_0)$? \tb{tbd}.





%Let $\mathcal{M}_{\Sigma} = \begin{bmatrix}\mathcal{M}_{\Sigma A} & \mathcal{M}_{\Sigma B} \end{bmatrix}$. The reachable region can be over approximated by 
%\begin{align}
%\mathcal{R}_{k+1} = \mathcal{M}_{\Sigma A} \mathcal{R}_{k} + \mathcal{M}_{\Sigma B} \mathcal{U} +  \mathcal{M}_w
%\end{align}
%

==> Sections/DAutomata_old.tex <==

\subsection{Automaton}
Automata is an appropriate model for the design and modeling discrete-event systems \cite{conf:automata1974,conf:introd2discrete}.  

\begin{definition}[\textbf{Automaton \cite{conf:matrixrep}}] \label{df:automata} 
An automaton is a tuple $A = (X,E,U,h,X0)$, where $X=\begin{bmatrix}x_1,\dots,x_n \end{bmatrix}$ is a finite set of state, $E$ a finite set of edges between states based on the input, $U=\begin{bmatrix}u_1,\dots,u_m \end{bmatrix}$ a finite set of input symbols called the alphabet, $X0$ a set of initial states, and $h: X \times U \rightarrow 2^X$ with $2^X$ denotes the set of all subsets of X, that is, $h(x_i,u_j) \subseteq X$ whenever it is defined for all $i$ and $j$.
\end{definition}

We define the semi-tensor product as follows. 
\begin{definition}\label{def:semitensor}\textbf{(Semi-tensor product \cite{conf:semitensor})}
Given two matrices $M \in \mathbb{Z}^{m \times n}$ and $N  \in \mathbb{Z}^{p \times q}$, the semi-tensor
product, denoted by $\ltimes$, is defined as:
\begin{align}
    M \ltimes N = (M \otimes I_{s_1})( N \otimes I_{s_2}),
\end{align}
with $s$ as the least common multiple of $n$ and $p$, $s_1 =s/n$, and $s_1 =s/p$.
\end{definition}

\begin{remark}
We perform the multiplication between ($M \otimes I_{s_1}$) and ($N \otimes I_{s_2}$) in Definition \ref{def:semitensor} by ANDing the corresponding bits and ORing the results to avoid having number greater than one. 
\end{remark}

Furthermore, we define the  Minkowski semi-tensor product with a slight abuse for the notation. 
\begin{align}
    \mathcal{L}_1 \ltimes  \mathcal{L}_2 	&= \{z_1 \ltimes z_2| z_1\in \mathcal{L}_1, z_2 \in \mathcal{L}_2 \} 
\end{align}
We make use of the transition structure matrix $H = \begin{bmatrix}H_1,\dots,H_m \end{bmatrix}\in \mathbb{R}^{n \times m n}$  where
$H_i \in \mathbb{R}^{n \times n}$ is the adjacency matrix while considering only edges with $u_i$ as input, and
\begin{align}
    H_i^{(j,t)} = \begin{cases} 1 &\quad\text{if}\,\, x_t \in h(x_j,u_i),\\
    0 &\quad\text{else}.
    \end{cases}
\end{align}



The following lemma determines the next state based on the input and the current state.
\begin{lemma}[\!\!\cite{conf:matrixrep}]\label{lm:automatadynamics}
The dynamic of an automaton $A$ can be described by
\begin{align}
    x(k+1) = H \ltimes u(k) \ltimes x(k).
\end{align}
\end{lemma}


\begin{theorem}
\label{thm:semitensorproductzonotopes}
Given two logical matrix zonotopes $\mathcal{L}_1=\langle c_{\mathcal{L}_1},G_{\mathcal{L}_1} \rangle \in \mathbb{Z}^{m \times n}$ and $\mathcal{L}_2 = \langle c_{\mathcal{L}_2},G_{\mathcal{L}_2} \rangle \in \mathbb{Z}^{p \times q}$, the Minkowski semi-tensor
product can be over-approximated by $\mathcal{L}_{\ltimes}$: 
\begin{align}
    \mathcal{L}_1 \ltimes \mathcal{L}_2 &\subseteq \Big\langle c_{\mathcal{L}_{\ltimes}} ,G_{\mathcal{L}_{\ltimes}} \Big\rangle.
     \label{eq:nandmink}
\end{align}
where 
\begin{align}
    c_{\mathcal{L}_{\ltimes}} {=}& \Big(c_{\mathcal{L}_1} {\otimes} I_{s_1}\Big)\Big(c_{\mathcal{L}_2} {\otimes} I_{s_2}\Big) \\
    G_{\mathcal{L}_{\ltimes}} {=}& \Big\{\Big(c_{\mathcal{L}_1} {\otimes} I_{s_1}\Big) \Big(g_{\mathcal{L}_2}^{(1)}  {\otimes} I_{s_2} \Big),\dots,\!\!\Big(c_{\mathcal{L}_1} {\otimes} I_{s_1}\Big) \Big(g_{\mathcal{L}_2}^{(k_1)}  {\otimes} I_{s_2} \Big), \nonumber \\
    &\!\!\!\!\Big(g_{\mathcal{L}_1}^{(1)}  {\otimes} I_{s_1} \Big)\Big(c_{\mathcal{L}_2} {\otimes} I_{s_2}\Big) ,\dots,\!\!\Big(g_{\mathcal{L}_1}^{(k_1)}  {\otimes} I_{s_1} \Big)\Big(c_{\mathcal{L}_2} {\otimes} I_{s_2}\Big)\nonumber \\
    &\!\!\!\!\Big(g_{\mathcal{L}_1}^{(1)}  {\otimes} I_{s_1} \Big)\Big(g_{\mathcal{L}_2}^{(1)}  {\otimes} I_{s_2} \Big),\dots,\!\!\Big(g_{\mathcal{L}_1}^{(k_1)}  {\otimes} I_{s_1} \Big)\Big(g_{\mathcal{L}_2}^{(k_2)}  {\otimes} I_{s_2} \Big) \Big\}
\end{align}
 with $s$ as the least common multiple of $n$ and $p$, $s_1 =s/n$, and $s_1 =s/p$.
\end{theorem}

\begin{proof}
Choose $z \in \mathcal{L}_1 \ltimes \mathcal{L}_2$. Then, $\exists \beta_{\mathcal{L}_1},\beta_{\mathcal{L}_2}$ such that
\begin{align}
z {=}& \Big(c_{\mathcal{L}_1} \xorsum{i=1}{k_{\mathcal{L}_1}}  g_{\mathcal{L}_1}^{(i)} \beta_{\mathcal{L}_1}^{(i)} \Big) \ltimes \Big(c_{\mathcal{L}_2} \xorsum{i=1}{k_{\mathcal{L}_2}}  g_{\mathcal{L}_2}^{(i)} \beta_{\mathcal{L}_2}^{(i)}\Big) \nonumber \\
{=}& \bigg( \Big(c_{\mathcal{L}_1} \xorsum{i=1}{k_{\mathcal{L}_1}}  g_{\mathcal{L}_1}^{(i)} \beta_{\mathcal{L}_1}^{(i)} \Big) \otimes I_{s_1} \bigg)  \bigg( \Big(c_{\mathcal{L}_2} \xorsum{i=1}{k_{\mathcal{L}_2}}  g_{\mathcal{L}_2}^{(i)} \beta_{\mathcal{L}_2}^{(i)} \Big) \otimes I_{s_2} \bigg) \nonumber \\
{=}& \Big(c_{\mathcal{L}_1} {\otimes} I_{s_1} \xorsum{i=1}{k_{\mathcal{L}_1}}  g_{\mathcal{L}_1}^{(i)} \beta_{\mathcal{L}_1}^{(i)} {\otimes} I_{s_1} \Big) \Big(c_{\mathcal{L}_2} {\otimes} I_{s_2} \xorsum{i=1}{k_{\mathcal{L}_2}}  g_{\mathcal{L}_2}^{(i)} \beta_{\mathcal{L}_2}^{(i)} {\otimes} I_{s_2} \Big) \nonumber \\
{=}& \Big(c_{\mathcal{L}_1} {\otimes} I_{s_1}\Big)\Big(c_{\mathcal{L}_2} {\otimes} I_{s_2}\Big) \xorsum{i=1}{k_{\mathcal{L}_2}} \Big(c_{\mathcal{L}_1} {\otimes} I_{s_1}\Big) \Big(g_{\mathcal{L}_2}^{(i)} \beta_{\mathcal{L}_2}^{(i)} {\otimes} I_{s_2} \Big) \nonumber \\
&\!\!{+}\xorsum{i=1}{k_{\mathcal{L}_1}}  \Big(g_{\mathcal{L}_1}^{(i)} \beta_{\mathcal{L}_1}^{(i)} {\otimes} I_{s_1} \Big) \Big(c_{\mathcal{L}_2} {\otimes} I_{s_2}\Big)\nonumber \\
&\!\!{+}\xorsum{i=1,j=1}{k_{\mathcal{L}_1},k_{\mathcal{L}_2}} \Big(g_{\mathcal{L}_1}^{(i)} \beta_{\mathcal{L}_1}^{(i)} {\otimes} I_{s_1} \Big) \Big(g_{\mathcal{L}_2}^{(j)} \beta_{\mathcal{L}_2}^{(j)} {\otimes} I_{s_2} \Big)
\label{eq:zZ1timeZ2} 
 \end{align}
 Combining the factors in $\beta_{\mathcal{L}_{\ltimes}} = \{ \beta_{\mathcal{L}_1},   \beta_{\mathcal{L}_2}, \beta_{\mathcal{L}_1} \beta_{\mathcal{L}_2} \}$ results in having $z \in \mathcal{L}_{\ltimes}$ and thus $\mathcal{L}_1 \ltimes \mathcal{L}_2 \subseteq \mathcal{L}_{\ltimes}$.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[scale = 0.2]{Figures/automata.png}
    \caption{Automaton example \cite{conf:matrixrep}.}
    \label{fig:my_label}
\end{figure}

Given we are able to over-approximate the semi-tensor product of two zonotopes, the reachable sets in an automaton given a state logical zonotope $\bar{\mathcal{R}}_k$ (or reachable set at time $k$) that contains the uncertain starting states $x_i \in \bar{\mathcal{R}}_k, \forall i=\{1,\dots,p_x\}$ and a input logical zonotope $\mathcal{L}_x$ that contains the uncertain inputs $u_i \in \mathcal{U}_k, \forall i=\{1,\dots,p_u\}$ can be described as follows:
\begin{theorem}
Given an automaton with a transition structure matrix $H$, reachable set $\bar{\mathcal{R}}_k$, and input logical zonotope $\mathcal{U}_k$, then next reachable set computed as
\begin{align}
    \bar{\mathcal{R}}_{k+1} \subseteq H \ltimes \mathcal{U}_k  \ltimes \bar{\mathcal{R}}_k.
\end{align}
over-approximates the exact reachable set, i.e., $\bar{\mathcal{R}}_{k+1} {\supseteq} \mathcal{R}_{k+1}$.
\end{theorem}
\begin{proof}
The proof follows immediately from Theorem \ref{thm:semitensorproductzonotopes} and Lemma \ref{lm:automatadynamics}.
\end{proof}

\begin{example}
 Consider an automaton $A {=} (X,E,U,h,X0)$ with $X{=}\{x_1,x_2,x_3,x_4,x_5\}$, $U{=}\{u_1,u_2,u_3,u_4\}$, $X0{=}x_1$ and transition structure matrix $H=\{H_1,H_2,H_3,H_4\}$ as follows:
 \begin{align}
     H  {=} \begin{bmatrix} 
      \begingroup % keep the change local
\setlength\arraycolsep{1.5pt}
     \begin{matrix} 
     0& 0 & 0 & 0& 0 \\
     1& 0 & 0 & 0& 0 \\
     0& 0 & 0 & 0& 0 \\
     0& 0 & 1 & 0& 0 \\
     0& 0 & 0 & 0& 0
     \end{matrix}
          \endgroup
     &
     \begingroup
     \setlength\arraycolsep{1.5pt}
     \begin{matrix}
     0 &0& 0& 0& 0  \\
     0& 0 & 0 & 0& 0 \\
     0& 1 & 0 & 0& 0 \\
     0& 1 & 0 & 0& 0 \\
     0& 0 & 0 & 0& 0
     \end{matrix} 
     \endgroup
         &
     \begingroup
     \setlength\arraycolsep{1.5pt}
     \begin{matrix}
     0 &0& 0& 0& 0  \\
     0& 0 & 0 & 0& 0 \\
     0& 0 & 1 & 0& 0 \\
     0& 1 & 0 & 0& 0 \\
     0& 0 & 0 & 0& 0
     \end{matrix} 
     \endgroup
              &
     \begingroup
     \setlength\arraycolsep{1.5pt}
     \begin{matrix}
     0 &0& 0& 0& 0  \\
     0& 0 & 0 & 0& 0 \\
     0& 0 & 0 & 0& 0 \\
     0& 0 & 0 & 0& 0 \\
     0& 0 & 1 & 1& 0
     \end{matrix} 
     \endgroup
     \end{bmatrix}
 \end{align}
 Consider uncertain starting states $\{x_3,x_4\}$ and uncertain control inputs $\{u_1,u_4\}$. We first compute using Lemma \ref{lm:enclosepoints} the state zonotope $\begingroup \setlength\arraycolsep{1.5pt} \bar{\mathcal{R}}_0=\zono{\begin{bmatrix} 1 & 0 & 0 & 0\end{bmatrix}^\top, \begin{bmatrix} 0 & 0 & 1 & 1\end{bmatrix}^\top }\endgroup$ which contains the starting states, and the input zonotope $\begingroup \setlength\arraycolsep{1.5pt} \mathcal{U}_0=\zono{ \begin{bmatrix} 0 & 0 & 0 & 1\end{bmatrix}^\top, \begin{bmatrix} 1 & 0 & 0 & 1\end{bmatrix}^\top }\endgroup$ which contains the uncertain control inputs. Then, we can compute using Theorem  \ref{thm:semitensorproductzonotopes} $\bar{\mathcal{R}}_1$
 \begin{align}
 \begingroup \setlength\arraycolsep{1.5pt}
 \bar{\mathcal{R}}_1 =\zono{\begin{bmatrix} 0 \\ 0 \\ 0 \\ 0 \\ 1 \end{bmatrix},\begin{bmatrix} 0 \\ 0 \\ 0 \\ 0 \\ 1 \end{bmatrix}  \begin{bmatrix} 0 \\ 0 \\ 0 \\ 1 \\ 1 \end{bmatrix} }
 \endgroup
 \end{align}
which if evaluated results in states $x_4$ and $x_5$. 
\end{example}

% \subsection{Execution Time}

% We generated a random automaton with $n=800$ states and input alphabet of size $m=100$. The of size of the transition structure matrix H is $800 \times 80000$. Consider that we want to find the next of states if we start from $p_x$ states while considering $p_u$ inputs from input alphabet. We computed the execution times in seconds and plotted them in Figure \ref{fig:execTimeGraph}. 


% \begin{figure}
%     \centering
%     \includegraphics[scale = 0.27]{Figures/execTimeGraph.eps}
%     \caption{The execution time in seconds with respect to different number of starting states and set of input for a automaton with $n=800$ states and input alphabet of size $m=100$.}
%     \label{fig:execTimeGraph}
% \end{figure}

==> Sections/oldEval.tex <==
\begin{comment}
\subsection{Reachability Analysis in Pursuit-Evasion Problem}
% states of the BCN from KTH paper
In a pursuit evasion problem in a polygonal environment, let there be $N$ regions. We define $3N$ state nodes in a BCN: $l_i(k) = \begin{bmatrix} 1 & 0 \end{bmatrix}^\top$ if pursuer located in region $i$ at time $k$, $v_i(k) = \begin{bmatrix} 1 & 0 \end{bmatrix}^\top$ if region $i$ visible by a pursuer at time $k$, $c_i(k) = \begin{bmatrix} 1 & 0 \end{bmatrix}^\top$ if region $i$ has already been cleared by a pursuer at time $k$. We write state $x(k) = (\ltimes_{i=1}^N l_i(k)) \ltimes (\ltimes_{i=1}^N v_i(k)) \ltimes (\ltimes_{i=1}^N c_i(k))$. 

% meta-variables of BCN (visible set, neighbor set)
From region $i$, the set of theoretically visible region indices is $\mathcal V_i$ and the set of neighbor region indices is $\mathcal N_i$. We assume there is uncertainty in whether other regions are visible or not. In other words, at time $k$, for theoretically visible region $j \in \mathcal V_i$, $v_j(k) \in \{\begin{bmatrix} 1 & 0 \end{bmatrix}^\top, \begin{bmatrix} 0 & 1 \end{bmatrix}^\top\}$ (it could be either visible or not visible). 

% inputs of the BCN
Let there be $P$ pursuers. Then, we have $PN$ input nodes in the BCN, $u^p_i(k) = \begin{bmatrix} 1 & 0 \end{bmatrix}^\top$ if pursuer $p$ enters into region $i$ at time $k$. We write input $u(k) = \ltimes_{p = 1}^P \ltimes_{i=1}^N u_i^p(k)$.
% input constraints how u(k) is selected
Each pursuer can only move to a neighbor region from time $k$ to $k+1$. In other words, for each pursuer $p$, the constraints on the selection of $u(k)$ is described by
\begin{align*}
    %\bigwedge_{i = 1 \ldots N} \left(u^p_i(k) \wedge \left(\bigwedge_{j \neq i} \neg u^p_j(k)\right)\right) = \begin{bmatrix} 1 \\ 0 \end{bmatrix} \\
    \forall i=1 \ldots N, \ u^p_i(k-1) \rightarrow \bigvee_{n \in \mathcal N_i} (u^p_n(k)=1) = \begin{bmatrix} 1 \\ 0 \end{bmatrix}
\end{align*}
Using $u(k)$, we can compute the set of possible $u(k+1)$'s.

% dynamics of BCN
The dynamics of the state nodes are described by
\begin{align}
    l_i(k+1) & = \bigvee_{p=1\ldots P} u^p_i(k) \\
    v_i(k+1) & = \bigvee_{v \in \mathcal V_i} l_v(k)  \\
    c_i(k+1) & = v_i(k) \vee \bigwedge_{n \in \mathcal N_i} (v_n(k) \vee c_n(k))
\end{align}

The dynamics of the pursuit-evasion problem is written as 
\begin{equation}
    x(k+1) = L \ltimes u(k) \ltimes x(k)
\end{equation}

% Figure of particular example
We use same layout as Figure 1 in "A Boolean Control Network Approach to Pursuit Evasion Problems in Polygonal Environments"~\cite{thunberg2011boolean}.

% initial condition
As an initial condition, we set the following to true,
\begin{equation}
    l_{21}(0) = \begin{bmatrix}1 \\ 0\end{bmatrix},\
    l_{15}(0) = \begin{bmatrix}1 \\ 0\end{bmatrix},\
    l_{12}(0) = \begin{bmatrix}1 \\ 0\end{bmatrix}
\end{equation}
and the rest of the state and input variables at $k=0$ to $\begin{bmatrix}0 & 1\end{bmatrix}^\top$ (false).

% result of reachability analysis
Then, we show the computation of $\hat{\mathcal R}_k$ for $k=1, 2, 3, 4$.

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{Figures/pursuit_example.pdf}
    \caption{\textcolor{red}{todo}}
    \label{fig:pursuit}
\end{figure}

\end{comment}


